On the boundary of the region defined by homomorphism densities

The Kruskal-Katona theorem together with a theorem of Razborov determine the closure of the set of points defined by the homomorphism density of the edge and the triangle in finite graphs. The boundary of this region is a countable union of algebraic curves, and in particular, it is almost everywhere differentiable. One can more generally consider the region defined by the homomorphism densities of a list of given graphs, and ask whether the boundary is as well-behaved as in the case of the triangle and the edge. Towards answering this question in the negative, we construct examples which show that the restrictions of the boundary to certain hyperplanes can have nowhere differentiable parts.

==> header.tex <==

\usepackage[margin=2cm]{geometry}   % set margin = 2cm
%\usepackage[dvipdfm]{hyperref}
\usepackage{url}
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs}
%\usepackage{natbib} % to use INFORMS bib style
\usepackage{enumerate}

\renewcommand{\baselinestretch}{1} % set spacing = 1.5 of the original spacing

%\topmargin 0pt
%\oddsidemargin 12pt
%\evensidemargin 12pt

%\textwidth 150mm
%\textheight 229mm

%\newtheorem{theorem}{Theorem}
\newtheorem{problem}{Problem}
\newtheorem{note}{Note}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}%[section]
%\newtheorem{proposition}{Proposition}%[section]
%\newtheorem{conj}{Conjecture}
%\theoremstyle{definition}
%\newtheorem{definition}{Definition}
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\numberwithin{equation}{section}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcM}{\mathcal{M}_\sigma}
\newcommand{\expect}{\mathbb{E}}
%\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
%\newcommand{\inp}[2]{\langle#1, #2\rangle}

\newcommand{\vect}[1]{\mathbf{#1}}

\renewcommand{\[}{\begin{equation}}
\renewcommand{\]}{\end{equation}}

\newcommand{\Int}{\mathrm{Int}}

\newcommand{\restate}[2]{\medskip
\noindent{\bf #1 (restated).}{\sl #2}}

\DeclareMathOperator{\Stab}{Stab}
%\DeclareMathOperator{\Prob}{Pr}
\DeclareMathOperator{\indx}{Ind}

\def\lc{\mathrm{lc}}
\def\cM{\mathcal{M}}
\def\cI{\mathcal{I}}
\def\cx{\mathbf{x}}

\def\poly{\mathrm{Poly}}

\definecolor{Blue}{rgb}{0,0,1}\def\blue{\color{Blue}}


